Split to Merge: Unifying Separated Modalities for Unsupervised Domain Adaptation

Large vision-language models (VLMs) like CLIP have demonstrated good zero-shot learning performance in the unsupervised domain adaptation task. Yet, most transfer approaches for VLMs focus on either the language or visual branches, overlooking the nuanced interplay between both modalities. In this work, we introduce a Unified Modality Separation (UniMoS) framework for unsupervised domain adaptation. Leveraging insights from modality gap studies, we craft a nimble modality separation network that distinctly disentangles CLIP's features into language-associated and vision-associated components. Our proposed Modality-Ensemble Training (MET) method fosters the exchange of modality-agnostic information while maintaining modality-specific nuances. We align features across domains using a modality discriminator. Comprehensive evaluations on three benchmarks reveal our approach sets a new state-of-the-art with minimal computational costs. Code: https://github.com/TL-UESTC/UniMoS

==> sec/3_finalcopy.tex <==
\section{Method}
Throughout this work, we adopt superscripts to distinguish domains. Symbols without a superscript are from both domains. Given a labeled source domain $\mathcal{D}^s=\{(x_i^s,y_i^s)\}_{i=1}^{N^s}$, the goal is to train a generalizable model that works well on the unlabeled target domain $\mathcal{D}^t=\{(x_i^t)\}_{i=1}^{N^t}$.
CLIP~\cite{clip} consists a vision encoder $g_{vis}$ and a text encoder $g_{txt}$. Given an image input $x$, CLIP-extracted vision feature is obtained by $f_v=g_{vis}(x)$. We follow the zero-shot inference paradigm in~\cite{padclip} to design naive prompts $\{(t_i)\}_{i=1}^K$ as ``a [DOMAIN] photo of a [CLASS].'', where $K$ is class number, [DOMAIN] describes domain characteristics and [CLASS] is class name. We then obtain CLIP-extracted text features by $\mu_i=g_{txt}(t_i)$. By comparing $f_v$ and $\mu_i$, an image is classified into a category with which it has the largest cosine similarity:
\begin{equation}
    \hat{y}_{zs}=\underset{i}{\arg  \max} \; \cos(\mu_i, f_v).
    \label{zeroshot}
\end{equation}

%Given a source domain $s$ and a target domain $t$,
%let $x_V^s$ and $x_T^s$ denote the image and text embeddings from the source domain, while $x_V^t$ is the image embeddings from the target domain.
%The goal is to predict the class labels of $x_V^t$ given the trained model on $x_V^s$ and $x_T^s$.

\subsection{Problem formulation}
This paper address the covariant shift, i.e., the data distribution shift between $x_V^s$ and $x_V^t$.  
We assume such distribution shift stems from the modality gap \cite{jiang2023understanding}. Therefore, we decompose the classification problem by classifying the text class along with the visual class. \red{how to introduce VAC and LAC} More specifically, we consider $Y=\{Y_V, Y_T\}$, where $Y_V$ is obtained by the VAC and $Y_T$ is obtained by $LAC$.

In what follows, we detail our approach.

% Proposal of modality gap in VLMs by Liang \textit{et al.}~\cite{liang2022mind}.

% 1. The problem of UDA, Eq.4;
% 2. The modality gap of CLIP, Eq,5 ,
% 3. Our proposal Eq. 6~8

% Construct better modality structures based on modality gap in VLMs by Jiang \textit{et al.}~\cite{jiang2023understanding} 
% \red{taking inspirations from 13, we make assumption of $X^V,X^T$}. 

% Target domain generalization error by David \textit{et al.}~\cite{ben2010theory} (Theorem 1). 

% A typical classification problem includes 
\begin{align}
    % & P(X^s,Y) \neq P(X^t,Y), \\
    % & P(Y|X^s)P(X^s) \neq P(Y|X^t)P(X^t),\\ 
    % & P(Y|X^s)=(\neq)P(Y|X^t), \\
    % & P(X^s) \neq P(X^t) \\
    & P(Y|T^c,V) = P(Y|X^T, X^V)\\
    & P(Y|Y^T,Y^V)\\
    & P(Y^T|X^T, X^{V1}) \\
    & P(Y^V | X^{V2})
\end{align}

% \begin{equation}
%     \epsilon^t \leq \epsilon^s + d(X^s,X^t) + (\epsilon^s(h^*)+\epsilon^t(h^*)),
% \end{equation}
% where
% \begin{equation}
%     h^* = \arg \underset{h}{\min} \; \epsilon^s(h)+\epsilon^t(h).
% \end{equation}

\subsection{Modality Separation Networks}
We first introduce the modality separation networks. As depicted by \cref{fig2}, modality separation networks consist of two separators that disentangle CLIP-extracted vision features into LAC and VAC.  We denote the text separator as $G_{txt}$ and the vision separator as $G_{vis}$, and then LAC and VAC are obtained by $f_{lac}=G_{txt}(f_v)$, $f_{vac}=G_{vis}(f_v)$. Both separators are linear layers that do not change the dimension of $f_v$, i.e., $f_{vac} \in \mathbb{R}^{d_v}$, $f_{lac} \in \mathbb{R}^{d_v}$. Inspired by deep feature separation~\cite{bousmalis2016domain}, we adopt an orthogonal loss to keep LAC and VAC distantly distributed.
\begin{equation}
    \mathcal{L}_{ortho} = \|f_{lac}^{s} \cdot  {f_{vac}^{s}}^{\top } \|_{F}^{2} + \|f_{lac}^{t} \cdot  {f_{vac}^{t}}^{\top } \|_{F}^{2}.
    \label{ortho}
\end{equation}
Afterwards, we obtain outputs for LAC and VAC differently. VAC is sent to a linear classification network consisting of two linear layers $\Phi_{1} \in \mathbb{R}^{d_v \times d_b}$, $\Phi_2 \in \mathbb{R}^{d_b \times K}$, where $d_b$ is dimension of bottleneck feature (output of $\Phi_1$). We then obtain output of $f_{vac}$ via:
\begin{equation}
    f_b = \Phi_1 (f_{vac}), ~~ \hat{y}_{vac} = \Phi_2 (f_b).
\label{vac_hat}
\end{equation}

For text modality, we follow zero-shot inference paradigm of CLIP to classify LAC. We compute cosine similarity between LAC and CLIP-extracted text features of each class as logits:
\begin{equation}
    \hat{y}_{lac} = (\hat{l}_1, \hat{l}_2, \cdots \hat{l}_k), ~~ \hat{l}_i = \cos(\mu_{i}, f_{lac})/T. 
\label{lac_hat}
\end{equation}

\subsection{Modality-Ensemble Training}
We design a modality-ensemble training (MET) paradigm to fully exploit modality-specific information and cooperatively utilize them to make accurate predictions. 

For text modality, we aim to preserve the semantic information contained in pretrained CLIP. A typical classification algorithm converts a class into a discrete class index and optimize by cross entropy, pulling down prediction probabilities of  all negative classes. In contrast, pretrained VLMs can capture subtle and rich semantic details that are helpful to identify hard samples. To safeguard these details, we apply knowledge distillation to directly distill the output of zero-shot CLIP outputs to LAC. We first obtain zero-shot similarity scores from pretrained CLIP as teacher output for target data:
\begin{equation}
    y_{lac}^t = (l_1-\overline{l} , l_2-\overline{l}, \cdots, l_k-\overline{l}), ~~ l_i = \cos(\mu_{i}, f_{v}^t)/T,
\label{lac}
\end{equation}
where $\overline{l}= \frac{1}{K} \sum_{k=1}^{K} l_k$ is a normalization factor to rescale CLIP outputs. For target data, we distill teacher knowledge to LAC, and for source data we directly optimize a cross entropy loss using source labels. By combing \cref{lac_hat} and \cref{lac}, the training loss for LAC can be formulated as:
\begin{equation}
    \mathcal{L}_{lac} = \mathrm{KL}(\hat{y}_{lac}^t, \, y_{lac}^t) + \alpha \mathrm{CE}(\hat{y}_{lac}^s, \, y^s),
    \label{llac}
\end{equation}
where $\alpha$ is a hyperparameter controlling the effect of source data supervision, $\mathrm{KL}(\cdot,\cdot)$ is KL divergence and $\mathrm{CE}(\cdot,\cdot)$ is standard cross entropy loss.

For image modality, we focus on locality structure of vision representations~\cite{elpt,nrc}, that is, well-aligned vision representations should present high inter-class discriminability and compact intra-class distribution. However, CLIP-extracted vision features present very little of the above characteristics (see \cref{tsne_init} for more details). To promote locality structures in the learned VAC, we adopt a Kmeans-based deep clustering algorithm~\cite{deepcluster,shot} to obtain pseudo-labels for unlabeled target data. We first obtain clustering centroids for class $k$ by:
\begin{equation}
    \mu_k = \frac{\sum_{x^t} \delta_k (\mathrm{softmax} (\hat{y}_{mix}^t)) \cdot f_b^t}{\sum_{x^t} \delta_k (\mathrm{softmax} (\hat{y}_{mix}^t))},
    \label{centroid}
\end{equation}
where $\hat{y}_{mix}^t$ is mixed outputs from both modalities, and $\delta_k$ takes the $k_{th}$ logit. To reduce imbalanced text modality predictions distilled from CLIP, we adopt Approximated Controlled Direct Effect (ACDE)~\cite{debiaspl} to obtain debiased similarity scores $\tilde{y}_{lac}^t$ obtained from LAC:
\begin{align}
    & \tilde{y}_{lac}^t = \hat{y}_{lac}^t - \tau \log \hat{p}, \label{debias1} \\
    & \hat{p} \leftarrow m\hat{p} + (1-m)\frac{1}{B}\sum_{i=1}^{B}p_i,\label{debias2}
\end{align}
where $m$ is a fixed momentum, $\tau$ is a fixed debias factor, $B$ is batch size and $p_i=\mathrm{softmax}(\hat{y}_{lac}^t)$ is classification probability of LAC. Then we define the mixed outputs by:
\begin{equation}
    \hat{y}_{mix}^t=\lambda \cdot \hat{y}_{vac}^t + (1-\lambda) \cdot \hat{y}_{lac}^t,
    \label{mixup}
\end{equation}
where $\lambda$ is hyperparameter controlling mixup ratio. Finally, given any bottleneck feature $f_b$, we compute its cosine similarity with all centroids and select the closest class as its pseudo label:
\begin{equation}
    y_{vac}^t = \arg \underset{k}{\max} \, \cos(f_b^t, \mu_k).
    \label{cluster}
\end{equation}

A direct approach to utilize $y_{vac}^t$ is to supervise the training process of VAC on unlabeled target data. However, we observe little performance improvements brought by this approach. The reason is that $y_{vac}^t$ is obtained from outputs from both modalities as shown in \cref{centroid} and \cref{cluster}, thus its supervision may counteract with modality separation networks, resulting in poor separation effects. To resolve this, we propose to distinguish modality-specific components in $y_{vac}^t$ by introducing text modality outputs, and enforce VAC to focus on vision-specific parts. As depicted in \cref{fig2}, we adopt a weight generator $W$ that takes current VAC as input, and decide how much weight should be assigned to both modalities. If current training is dominated by text modality, vision outputs are assigned smaller weights to avoid destruction of VAC, and vice versa. To provide more flexibility for the ensemble strategy, we further propose to randomly reset half of the parameters of $W$ each epoch. Note that this only involves unlabeled target data. Formally, weighted ensemble outputs can be denoted as:
\begin{equation}
    \hat{y}_{ens}^t = w \cdot \hat{y}_{vac}^t + (1-w) \cdot \hat{y}_{lac}^t,
    \label{ensemble}
\end{equation}
where $w=W(VAC^t)$ is ensemble weight between 0 and 1. Notably, $y_{lac}^t$ in \cref{ensemble} is detached from the computation graph, thus does not affect the training of LAC. 

To promote better individual discriminability and global diversity that helps preserve and improve the locality structure of vision representations, we further apply information maximization loss~\cite{ahmed2021unsupervised,shot,hu2017learning} on $\mathcal{L}_{vac}$. We first define $\mathcal{L}_{ent}$ that improve individual certainty:
\begin{equation}
    \mathcal{L}_{ent} = -\mathbb{E}_{x^t \in X^t}[\sum_{k=1}^{K} \delta_k (\hat{y}_{ens}^t) \log \delta_k (\hat{y}_{ens}^t)],
\end{equation}
where $\delta_k$ takes the $k_{th}$ logit of ensemble outputs. We then define $\mathcal{L}_{div}$ that encourages diverse class distribution in ensemble outputs by:
\begin{equation}
    \mathcal{L}_{div} = -\sum_{k=1}^{K} \overline{l}_k \log \overline{l}_k, 
\end{equation}
where $\overline{l}_k=-\mathbb{E}_{x^t \in X^t} \delta_k(\hat{y}_{ens}^t)$. Overall information maximization loss $\mathcal{L}_{im}$ is defined as:
\begin{equation}
    \mathcal{L}_{im} = \mathcal{L}_{ent} - \mathcal{L}_{div}.
    \label{im}
\end{equation}
Finally, we supervise the training of $y_{ens}^t$ on vision modality target pseudo labels obtained via \cref{cluster}, and directly optimize $y_{vac}^s$ by source labels. The overall training loss of VAC is defined as:
\begin{equation}
    \mathcal{L}_{vac} = CE(\hat{y}_{ens}^t, \, y_{vac}^t) + \beta CE(\hat{y}_{vac}^s, \, y^s) + \mathcal{L}_{im},
    \label{lvac}
\end{equation}
where $\beta$ is a hyperparameter controlling the effect of source data supervision, and $\mathrm{CE}(\cdot,\cdot)$ is standard cross entropy loss. It should be noted that the ensemble weights $w$ in \cref{ensemble} is different from the mixup ratio $\lambda$ in \cref{mixup}. The former is learned dynamically during training process to decide appropriate weights that do not harm modality separation effects, while the latter is a constant hyperparameter for each sample each time we obtain pseudo labels, aiming to explore better pseudo labels by taking both modality-specific predictions into consideration. MET effectively exploits modality-specific information by optimizing LAC and VAC in different ways that best suit their modality, while exchanging modality-invariant information in a way that does harm the modality separation effect.

\subsection{Cross-Domain Modality Discriminator}
As shown in \cref{fig2}, we design a modality discriminator $D$ that aligns VAC and LAC from both domains while further enhances modality separation effects. The domain discriminator in adversarial domain adaptation methods~\cite{dann,cdan} tries to identify to which domain the features belong, promoting the extraction of domain invariant features via adversarial training. In multimodal domain adaptation, applying two separate domain discriminators for two modalities respectively is redundant and suboptimal, as they overlook the connections between the two modalities. We propose to train a single modality discriminator to distinguish between LAC and VAC on source domain, and apply it to target domain to measure whether the target LAC and VAC are aligned with source ones. If both modalities from both domains are well aligned, the modality discriminator should be able to correctly distinguish target LAC and VAC, even without being trained on target domain. We adopt binary cross entropy loss to train the modality discriminator:
\begin{equation}
    \mathcal{L}_{bce} = -[y_{dis} \log \hat{y}_{dis} + (1-y_{dis}) \log (1-\hat{y}_{dis})],
    \label{dis}
\end{equation}
where $y_{dis}$ is modality label, defined as 0 for VAC and 1 for LAC, and $\hat{y}_{dis}$ is discrimination result given by $D$. Note that modality discriminator $D$ is only optimized by \cref{dis} on source domain. On target domain, only the modality separators $G_{vis}, G_{txt}$ are updated to minimize \cref{dis}, so that target LAC and VAC are aligned with source ones.

\begin{algorithm}[t]
    \caption{Training Algorithm of CDMoS}
    \label{alg1}
    \textbf{Input}: Labeled source data ${x^s, y^s}$, unlabeled target data $x^t$, maximum epoch number $max\_epoch$, pretrained CLIP text encoder $g_{txt}$ and vision encoder $g_{vis}$.\\
    \textbf{Output}: Trained modality separator $G_{txt},G_{vis}$, and trained linear layers $\Phi_1,\Phi_2$.
    \begin{algorithmic}[1] %[1] enables line numbers
    \STATE Let $epoch=0$.
    \WHILE{$epoch < max\_epoch$}
    \STATE Obtain teacher output $y_{lac}^t$ via \cref{lac}.
    \IF {$epoch\mod2==0$}
    \STATE Take mixed outputs as target vision pseudo label via \cref{mixup}.
    \ELSE 
    \STATE Obtain target vision pseudo label $y_{vac}^t$ via \cref{cluster}.
    \ENDIF
    \STATE Randomly reset half of the parameters of $W$.
    \STATE Obtain CLIP-extracted vision $f_v=g_{vis}(x^s,x^t)$ and text features $\mu_i=g_{txt}(t_i)$.
    \STATE Obtain LAC outputs $\hat{y}_{lac}$ by \cref{lac_hat}.
    \STATE Obtain VAC outputs $\hat{y}_{vac}$ by \cref{vac_hat}.
    \STATE Obtain ensemble outputs $\hat{y}_{ens}$ by \cref{ensemble}.
    \STATE Obtain modality discrimination outputs $y_{dis}$ by \cref{dis}.
    \STATE Update network parameters via \cref{opt}.
    \ENDWHILE
    \STATE \textbf{return} solution
    \end{algorithmic}
\label{algorithm}
\end{algorithm}

\begin{table*}[ht]
    \caption{UDA results on Office-Home. Best results are marked in bold font. Methods with `*' are based on CLIP.}
    \vspace{-8pt}
    \centering
    \label{officehome}
    %\scriptsize
    %\begin{tabular}{c|c|c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c \hhs c|c}
    \resizebox{\linewidth}{!}{ 
    \begin{tabular}{c|c|cccccccccccc|c}
    \toprule
    %Method & Backbone & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & Avg. \\ \midrule
    Method & Backbone & A$\to$C & A$\to$P & A$\to$R & C$\to$A & C$\to$P & C$\to$R & P$\to$A & P$\to$C & P$\to$R & R$\to$A & R$\to$C & R$\to$P & Avg. \\ \midrule
    SourceOnly~\cite{resnet} & \multirow{15}{*}{ResNet50} & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
    ParetoDA~\cite{pareto} &  & 56.8 & 75.9 & 80.5 & 64.4 & 73.5 & 73.7 & 65.6 & 55.2 & 81.3 & 75.2 & 61.1 & 83.9 & 70.6 \\
    CLIP*~\cite{clip} &  & 51.7 & 81.5 & 82.3 & 71.7 & 81.5 & 82.3 & 71.7 & 51.7 & 82.3 & 71.7 & 51.7 & 81.5 & 71.8 \\
    SDAT~\cite{sdat} &  & 58.2 & 77.1 & 82.2 & 66.3 & 77.6 & 76.8 & 63.3 & 57.0 & 82.2 & 74.9 & 64.7 & 86.0 & 72.2 \\
    MSGD~\cite{msgd} &  & 58.7 & 76.9 & 78.9 & 70.1 & 76.2 & 76.6 & 69.0 & 57.2 & 82.3 & 74.9 & 62.7 & 84.5 & 72.3 \\
    Fixbi~\cite{fixbi} &  & 58.1 & 77.3 & 80.4 & 67.7 & 79.5 & 78.1 & 65.8 & 57.9 & 81.7 & 76.4 & 62.9 & 86.7 & 72.7 \\
    CST~\cite{cst} &  & 59.0 & 79.6 & 83.4 & 68.4 & 77.1 & 76.7 & 68.9 & 56.4 & 83.0 & 75.3 & 62.2 & 85.1 & 72.9 \\
    ATDOC~\cite{atdoc} &  & 60.2 & 77.8 & 82.2 & 68.5 & 78.6 & 77.9 & 68.4 & 58.4 & 83.1 & 74.8 & 61.5 & 87.2 & 73.2 \\
    KUDA~\cite{kuda} &  & 58.2 & 80.0 & 82.9 & 71.1 & 80.3 & 80.7 & 71.3 & 56.8 & 83.2 & 75.5 & 60.3 & 86.6 & 73.9 \\
    DAPL*~\cite{dapl} &  & 54.1 & 84.3 & 84.8 & 74.4 & 83.7 & 85.0 & 74.5 & 54.6 & 84.8 & 75.2 & 54.7 & 83.8 & 74.5 \\
    EIDCo~\cite{eidco} &  & \textbf{63.8} & 80.8 & 82.6 & 71.5 & 80.1 & 80.9 & 72.1 & 61.3 & 84.5 & \textbf{78.6} & \textbf{65.8} & 87.1 & 75.8 \\
    ICON~\cite{icon} &  & 63.3 & 81.3 & 84.5 & 70.3 & 82.1 & 81.0 & 70.3 & 61.8 & 83.7 & 75.6 & 68.6 & 87.3 & 75.8 \\
    ADCLIP*~\cite{adclip} &  & 55.4 & 85.2 & 85.6 & 76.1 & 85.8 & 86.2 & \textbf{76.7} & 56.1 & 85.4 & 76.8 & 56.1 & 85.5 & 75.9 \\
    PADCLIP*~\cite{padclip} &  & 57.5 & 84.0 & 83.8 & \textbf{77.8} & 85.5 & 84.7 & 76.3 & \textbf{59.2} & 85.4 & 78.1 & 60.2 & 86.7 & 76.6 \\
    \rowcolor[HTML]{d1cfcf} 
    CDMoS* (ours) &  & 59.5 & \textbf{89.4} & \textbf{86.9} & 75.2 & \textbf{89.6} & \textbf{86.8} & 75.4 & 58.4 & \textbf{87.2} & 76.9 & 59.5 & \textbf{89.7} & \textbf{77.9} \\ \midrule
    CDTrans~\cite{cdtrans} & DeiT-B & 68.8 & 85.0 & 86.9 & 81.5 & 87.1 & 87.3 & 79.6 & 63.3 & 88.2 & 82.0 & 66.0 & 90.6 & 80.5 \\ \midrule
    SourceOnly~\cite{vit} & \multirow{8}{*}{ViT-B} & 54.7 & 83.0 & 87.2 & 77.3 & 83.4 & 85.5 & 74.4 & 50.9 & 87.2 & 79.6 & 53.8 & 88.8 & 75.5 \\
    CLIP*~\cite{clip} &  & 67.8 & 89.0 & 89.8 & 82.9 & 89.0 & 89.8 & 82.9 & 67.8 & 89.8 & 82.9 & 67.8 & 89.0 & 82.4 \\
    TVT~\cite{tvt} &  & 74.9 & 86.8 & 89.5 & 82.8 & 88.0 & 88.3 & 79.8 & 71.9 & 90.1 & 85.5 & 74.6 & 90.6 & 83.6 \\
    DAPL*~\cite{dapl} &  & 70.6 & 90.2 & 91.0 & 84.9 & 89.2 & 90.9 & 84.8 & 70.5 & 90.6 & 84.8 & 70.1 & 90.8 & 84.0 \\
    SSRT~\cite{ssrt} &  & 75.2 & 89.0 & 91.1 & 85.1 & 88.3 & 89.9 & 85.0 & 74.2 & 91.2 & 85.7 & 78.6 & 91.8 & 85.4 \\
    ADCLIP*~\cite{adclip} &  & 70.9 & 92.5 & 92.1 & 85.4 & 92.4 & 92.5 & \textbf{86.7} & 74.3 & \textbf{93.0} & \textbf{86.9} & 72.6 & 93.8 & 86.1 \\
    PADCLIP*~\cite{padclip} &  & \textbf{76.4} & 90.6 & 90.8 & \textbf{86.7} & 92.3 & 92.0 & 86.0 & \textbf{74.5} & 91.5 & \textbf{86.9} & \textbf{79.1} & 93.1 & 86.7 \\
    \rowcolor[HTML]{d1cfcf} 
    CDMoS* (ours) &  & 74.9 & \textbf{94.0} & \textbf{92.5} & 86.4 & \textbf{94.3} & \textbf{92.5} & 86.0 & 73.9 & \textbf{93.0} & 86.4 & 74.2 & \textbf{94.5} & \textbf{86.9} \\ \bottomrule
    \end{tabular}}
  \end{table*}
  
  \begin{table*}[ht]
    \caption{UDA results on VisDA-2017. Best results are marked in bold font. Methods with `*' are based on CLIP.}
    \vspace{-8pt}
    \label{visda}
    \footnotesize
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|cccccccccccc|c}
    \toprule
    Method & Backbone & plane & bicycle & bus & car & horse & knife & mcycl & person & plant & sktbrd & train & truck & Avg. \\ \midrule
    SourceOnly~\cite{resnet} &  & 55.1 & 53.3 & 61.9 & 59.1 & 80.6 & 17.9 & 79.7 & 31.2 & 81.0 & 26.5 & 73.5 & 8.5 & 52.4 \\
    ParetoDA~\cite{pareto} &  & 95.9 & 82.8 & 81.3 & 58.7 & 93.9 & 93.7 & 85.9 & 83.0 & 91.9 & 92.0 & 87.1 & 51.8 & 83.2 \\
    CLIP*~\cite{clip} &  & \textbf{98.2} & 83.9 & 90.5 & 73.5 & 97.2 & 84.0 & 95.3 & 65.7 & 79.4 & 89.9 & 91.8 & 63.3 & 84.4 \\
    MSGD~\cite{msgd} &  & 97.5 & 83.4 & 84.4 & 69.4 & 95.9 & 94.1 & 90.9 & 75.5 & 95.5 & \textbf{94.6} & 88.1 & 44.9 & 84.5 \\
    ATDOC~\cite{atdoc} &  & 95.3 & 84.7 & 82.4 & 75.6 & 95.8 & 97.7 & 88.7 & 76.6 & 94.0 & 91.7 & 91.5 & 61.9 & 86.3 \\
    DAPL*~\cite{dapl} &  & 97.8 & 83.1 & 88.8 & 77.9 & 97.4 & 91.5 & 94.2 & 79.7 & 88.6 & 89.3 & \textbf{92.5} & 62.0 & 86.9 \\
    CAN~\cite{can} &  & 97.0 & 87.2 & 82.5 & 74.3 & 97.8 & \textbf{96.2} & 90.8 & 80.7 & 96.6 & 96.3 & 87.5 & 59.9 & 87.2 \\
    FixBi~\cite{fixbi} &  & 96.1 & 87.8 & 90.5 & \textbf{90.3} & 96.8 & 95.3 & 92.8 & \textbf{88.7} & \textbf{97.2} & 94.2 & 90.9 & 25.7 & 87.2 \\
    ADCLIP*~\cite{adclip} &  & 98.1 & 83.6 & \textbf{91.2} & 76.6 & \textbf{98.1} & 93.4 & \textbf{96.0} & 81.4 & 86.4 & 91.5 & 92.1 & 64.2 & 87.7 \\
    PADCLIP*~\cite{padclip} &  & 96.7 & \textbf{88.8} & 87.0 & 82.8 & 97.1 & 93.0 & 91.3 & 83.0 & 95.5 & 91.8 & 91.5 & 63.0 & \textbf{88.5} \\
    \rowcolor[HTML]{d1cfcf} 
    CDMoS* (ours) & \multirow{-11}{*}{ResNet101} & 97.7 & 88.2 & 90.1 & 74.6 & 96.8 & 95.8 & 92.4 & 84.1 & 90.8 & 89.0 & 91.8 & \textbf{65.3} & 88.1 \\ \bottomrule
    \end{tabular}}
    \vspace{-8pt}
  \end{table*}

\subsection{Training Algorithm}
We first give optimization objectives of our method. As depicted in \cref{fig2}, the pretrained text encoder and vision encoder are frozen, and we  optimize parameters of $G_{txt}$, $G_{vis}$, $\Phi_1$, $\Phi_2$, $W$, $D$, denoted as $\theta_{G_{txt}}$, $\theta_{G_{vis}}$, $\theta_{\Phi_1}$, $\theta_{\Phi_2}$, $\theta_{W}$, $\theta_{D}$, respectively. Combining \cref{llac}, \cref{im}, \cref{ortho}, \cref{lvac}, \cref{dis}, we define the following optimization problem.
\begin{align}
    & \theta_{G_{txt}} = \underset{\theta_{G_{txt}}}{\arg \min} \; \mathcal{L}_{lac} + \gamma\mathcal{L}_{ortho} + \gamma\mathcal{L}_{bce}, \label{opt}\\
    & \theta_{G_{vis}} = \underset{\theta_{G_{vis}}}{\arg  \min} \; \mathcal{L}_{vac} + \gamma\mathcal{L}_{ortho} + \gamma\mathcal{L}_{bce}, \nonumber \\
    & \theta_{W}, \, \theta_{\Phi_1}, \, \theta_{\Phi_2} = \underset{\theta_{W},\theta_{\Phi_1},\theta_{\Phi_2}}{\arg \min} \; \mathcal{L}_{vac}, \nonumber \\
    & \theta_{D} = \underset{\theta_{D}}{\arg \min} \; \gamma \mathcal{L}_{bce} \nonumber ,
\end{align}
where $\gamma$ is weight for regularization terms $\mathcal{L}_{bce}$ and $\mathcal{L}_{ortho}$. We then present detailed training procedure of CDMoS in \cref{algorithm}. Note that in lines 4$\sim$7, we propose to replace $y_{vac}^t$ used in \cref{lvac} by mixed outputs in \cref{mixup} in certain epochs, in order to avoid error accumulation~\cite{decorate} in vision pseudo labels.

